SmartAnnotator: An Interactive Tool for Annotating RGBD Indoor Images

RGBD images with high quality annotations in the form of geometric (i.e., segmentation) and structural (i.e., how do the segments are mutually related in 3D) information provide valuable priors to a large number of scene and image manipulation applications. While it is now simple to acquire RGBD images, annotating them, automatically or manually, remains challenging especially in cluttered noisy environments. We present SmartAnnotator, an interactive system to facilitate annotating RGBD images. The system performs the tedious tasks of grouping pixels, creating potential abstracted cuboids, inferring object interactions in 3D, and comes up with various hypotheses. The user simply has to flip through a list of suggestions for segment labels, finalize a selection, and the system updates the remaining hypotheses. As objects are finalized, the process speeds up with fewer ambiguities to resolve. Further, as more scenes are annotated, the system makes better suggestions based on structural and geometric priors learns from the previous annotation sessions. We test our system on a large number of database scenes and report significant improvements over naive low-level annotation tools.

==> comments.tex <==
Comments by James
Q: What is scene labeling?
A: To label everything in a scene (indoor/outdoor)

Q: How does it do?
A: good features + large training data + supervised learning

Q: What are the existing efforts?
A: focus on designing image features

why we use cuboid layout and related features to train probabilistic models?
because it could obtain better labeling accuracy?







Niloy:
problem: annotating RGBD data
    1. segmentation; 2. labeling; 3. inter-relations -- contact, support, occlusions ..
challenges:
    1. data quality; occlusion; missing parts ...
solution:
    1. priors in the form of mixture models
    2. context .. structure ..
    3. priors both for size, and also arrangement/structure
we ignore color, texture ..
user interacts by scribble of boxes/selection of labels in 2D, but algorithm works/reasons in 3d
we also have priors of objects from 3d benchmarks (ikea, etc.)
progressive performance .. easier as some parts are correctly labelled
interface + user experience

user experience:
1. user selects some boxes or we get ransac to create some boxes
2. system suggests labels for each box + user approves label for the most confident box
3. next box lbael suggestions are updated and presented to the user ..
4. based on the selected label, the box dimensions are refined and labels for all remaining boxes reestimated ..we iterate until all boxes are labeled
final output: segments, boxes, labels, contact graph (structure)

%
reference
1. Semantic Labeling of 3D Point Clouds for Indoor Scenes:
RGB-D
Require a full point cloud model to capture enough information.
captures various features and contextual relations, including the local visual appearance and
shape cues, object co-occurence relationships and geometric relationships.


2. Hedau et al. [19] Thinking inside the box: Using appearance models and context based on room geometry
recovers the 3D structure of the room from
a single image, which then provides context for recognition.

3.G. Csurka, C. Dance, L. Fan, J. Willamowski, and C. Bray. Visual categorization with bags of keypoints.
In Workshop on statistical learning in computer vision, ECCV, 2004.
features: bag of words

4.N. Dalal and B. Triggs. Histograms of oriented gradients for human detection. In CVPR, 2005.
features: HOG

5. A. Torralba. Contextual priming for object detection. IJCV, 53(2):169???191, 2003.
features: GIST

6. X. Xiong and D. Huber. Using context to create semantic 3d models of indoor environments. In BMVC,2010.
label the planar patches in a point-cloud of an
indoor scene with four geometric labels (walls, floors, ceilings, clutter). They use a CRF to model
geometrical relationships such as orthogonal, parallel, adjacent, and coplanar. T

7. N. Silberman, D. Hoiem, P. Kohli, and R. Fergus. Indoor segmentation and support inference from RGBD images. In ECCV, 2012.
NYU RGB-D dataset V2
 In other recent works, Silberman et al. [23] identify which image segments support which other segments.
However, reasoning about support and stability are two different things.


8. Gupta, A., Efros, A.A., Hebert, M.: Blocks world revisited: Image understanding
using qualitative geometry and mechanics. In: ECCV. (2010)

9.Russell, B.C., Torralba, A.: Building a database of 3d scenes from user annotations.
In: CVPR. (2009)
show how a dataset of user-annotated scenes can be used to infer 3D structure and support

10.Zhang, C., Wang, L., Yang, R.: Semantic segmentation of urban scenes using dense
depth maps. In: ECCV. (2010)

11. Silberman, N., Fergus, R.: Indoor scene segmentation using a structured light sensor.
NYU RGB-D dataset

12. SUN3D???A Database of Big Spaces Reconstructed using SfM and Object Labels
SUN3D

13. 3D-Based Reasoning with Blocks, Support, and Stability

14. WordNet

Comments by Tirth

1. simultaneous capture and learning
   ref : globFit
   niloy has presented some point about this topic at siggraph11
   http://encore.siggraph.org/members/presentation11.asp?presId=116

2. middle layer abstraction
    in last decade, instead of use low level feature to do recognition and learning,
    we have seen how CV community use middle layer abstraction to improve the prediction. ...

    ref:  relative attributes, (Kristen Grauman's group)
    source ref:  Beyond Nouns: Exploiting Prepositions and Comparative Adjectives for Learning

3. geometry proxy
    In this work, we use a geometry proxy layer as the another abstraction..
   ...this introduce several benefit ... (ref following (4. & 5.) )

     ref: siggraph asia 2012 scene papers

4. global prediction/capture and interactive prediction
    in our framework, instead of recognition single object, we do prediction on all boxes at the same time
    ( maybe we could bring some point/challenge of task from holistic scene understanding paper)
    http://www.cs.cornell.edu/~asaxena/ccm/feccm_eccv2010.pdf
     http://vision.stanford.edu/documents/LiSocherFei-Fei_CVPR2009.pdf
    http://ai.stanford.edu/~koller/Papers/Heitz+al:NIPS08a.pdf

5.  structure output
    since we have the geometry proxy, our output is much richer.
    compare to indoor support inferring paper in ECCV'12 , alought they already have NYU V2, they still need human to do
    labeling the support relationship about each super pixel.
    this is another cost.
    but in our framework, we can infer this directly from our geometry proxy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if 1
%
Scene labeling, the process to label objects in a scene, is a fundamental
problem to scene understanding in the field of computer vision.
%
In recent years, a remarkable progress has been made in a challenging
task of labeling indoor scenes which involve large variation in
scene types, diversity of object categories, and heavy occlusion among
objects in a cluttered scene.
%
Most works has devoted to explore various 2D features extracted from a
set of labeled ground truth image which are further used to train a
probabilistic model for performing the labeling task.~\cite{}
%
The popularity of affordable {\rgbd} sensors (e.g. Microsoft Kinect) that
provide synchronized color and depth data has renewed the perspective of
traditional indoor scene labeling and significantly improved the
performance by incorporate 3D features inferred from {\rgbd} images~\cite{}.
%
However, to a robust scene labeling system, these approaches face a common
problem of working upon a small amount of labeled training data and the
burden of extending such dataset is completely laying on manual labor from
user.
%


To ease the problem, Russell~\etal~\shortcite{Russell:08:Label} developed
LabelMe, the most commonly used web-based image annotation tool, to provide
user an easy-to-use drawing interface to collaboratively annotate objects.
%
It allows user to annotate object by drawing polygonal outlines followed
by freely typing in the object label.
%
However, such drawing-based tool still demands tremendous manual efforts
and provides little information of object labels and segmentations in the
labeled image.
%
Therefore it poorly scales up with the available data, in particular for
indoor scenes where images usually contain cluttered objects with
complex boundaries and occlusions.
%

Our goal is to create an indoor image annotation system that requires minimal
manual efforts from user and is able to extract rich geometric and contextual
information from the annotated image.
%
For this purpose, we integrate a supervised learning algorithm with the object
annotating tasks and exploit the geometric and contextual priors learned from
the labeled datasets to infer object labels, segmentations and inter-object
relations including supporting hierarchy and occlusions.
%
In contrast to traditional tools which require tremendous labor from user to
manually annotate object labels and segmentations, our system allows user to
focus on supervising the information inferred by machine and assisting the
machine to progressively improve its performance by correcting a few object
labels.

%
%The key to improve the situation is a novel annotating system that could
%lighten the manual burden and interact with user in a simple, fast, and most importantly, smart way.
%In general, researches in indoor scene labeling are agreed in a principled
%flow of extracting features from a set of labeled ground truth images to
%serve as training data for a supervised learning algorithm.
%And two state-of-the-art 3D datasets, the NYU depth
%dataset~\cite{silberman:12:indoor} and SUN3D~\cite{Xiao:13:SUN3D}, are built
%to capture and support large amount of {\rgbd} indoor images.
%
%
%

We observed that although it is evident a good labeled dataset and a robust scene labeling system
are tightly coupled, each of them is considered in isolation.

%
It has been proven that while the combination of appearance features (e.g. SHIFT and HOG) and depth data along may already achieve impressive labeling accuracy~\cite{silberman:11:indoor}, a dramatic performance gains could be obtained by introducing high level contextual relations~\cite{Ren:12:RGBD,silberman:12:indoor,koppula:11:semantic}.

It is well-recognized that the keys to a robust scene labeling algorithm comprised of two parts.
%
The first one is how to design good features for a supervised learning algorithm and the other is the
ability to provide as many labeled ground truth images to serve as training data.
%
While a remarkable progress has been made in the first part~\cite{},
the burden of generating labeled training data completely lay on manual labor from users.
%
To ease the problem, Russell~\etal~\shortcite{Russell:08:Label} developed LabelMe, the most commonly used
web-based image annotation tool, that provides users an easy-to-use drawing interface to collaboratively
annotate objects by drawing polygonal outlines and allows user to freely type in the object label.
%
However, such drawing-based tool still demands tremendous manual efforts and therefore poorly scales up with
the available data, in particular for indoor scenes where images usually contain cluttered objects with
complex boundaries and occlusions.


The popularity of affordable {\rgbd} sensor has motivated a renewed interest in indoor scene labeling~\cite{Ren:12:RGBD,silberman:11:indoor,silberman:12:indoor}
which further introduce new publically available
%

%% we focus on annotating {\rgbd} images
%% require minimal manual effort while provide rich contextual information
%% the challenges:  infer rich geometric and contextual information
In this paper, we present an interactive annotation tool that focuses on annotating {\rgbd} indoor images.
%
In contrast to traditional annotation tools that solely rely on heavy labor from users to provide common
data such as labels and segmentations via a drawing interface, we aim at a system that requires minimal
manual efforts to obtain, in addition to common data, extra rich geometric and contextual information in the
annotated results.
%

It is well-recognized that the answer to the question "how to apply supervised learning algorithm on a
set of good features extracted from a sufficiently large and reliable dataset of labeled ground truth images"
plays the key role to a robust scene labeling algorithm.

The ability to collect a large dataset of labeled ground truth images has been recognized as one of key
components to obtain dramatic performance gains in scene labeling researches.
%
Most works in scene labeling require an input dataset with labeled objects from which they extract various
features and apply supervised learning to perform tasks such as and is used to qualitatively evaluate
the performance.
%
Although a remarkable progress has been made, a majority of research focused on design good features
and novel learning models to increase performance gains while merely build up on existing image databases
with limited collection of labeled images.
%

There is few works targeting on an effective tool to facilitate the annotation process while offering reliable and rich information
that would therefore benefit potential applications.
%

This is partly because the current image annotation tools, e.g. LabelMe~\cite{Russell:08:Label}, still require
tremendous manual efforts from users to annotate objects through a drawing-based interface and is therefore
difficult to scale up with the available data.
%
For instance, in indoor scene labeling where images usually contain cluttered objects with complex boundaries
and occlusions, it becomes a tedious process for users to one by one draw polygonal outlines on objects and
type in the labels, not even mentioning the quality of drawn polygon boundaries.
%
Moreover, results generated by such drawing-based tools contain only simple information
%

The process to label objects in a scene, also refers to scene labeling,
is a fundamental part to scene understanding in computer vision.
%
While a remarkable progress has been made in the outdoor scene labeling~\cite{},
a majority of research efforts have recently focused on a challenging task of
indoor scene labeling~\cite{} which involves large variation in scene types, diversity
of object categories, and heavy occlusion among objects in a cluttered scene.
%
In general, most works in indoor scene labeling require an input dataset of images
with ground truth object labels from which they could extract various features for
supervised learning and is used to qualitatively evaluate the performance.
%
However, many approaches aim to design good features and novel learning models
to obtain performance gains and usually build up on existing image databases with limited
collection of labeled images.
%
Even though it is recognized that a dramatic performance gains could be obtained as more
labeled training data is made available, there is few works emphasizing on an effective way
to expand the collection of labeled images.



To collect a large dataset of labeled images, Russell~\etal~\shortcite{Russell:08:Label}
developed the state-of-the-art web-based image annotation tool, called LabelMe, allowing
a large population of users to collaboratively annotate images and share the collection instantly.
%
It provides user an easy-to-use drawing interface to annotate object at different level of complexity
by drawing polygonal outline on object or its part, and allows user to freely type in the object name.
%
The simplicity and flexibility of LabelMe has made it nowadays a popular annotation tool used in many
research fields of computer vision and machine learning that demand a large dataset of labeled images.
%
However, in certain application such as indoor scene labeling in particular, images might contain
cluttered objects with complex boundaries, and user is asked to accurately outline the object contours
in order to obtain a reliable labeled dataset.
%
Using drawing-based interface will add tremendous burden on user, making even labeling a single image
a tedious process and is difficult to scale up with available data.

%
Our system starts by training classifiers using geometric priors and the structural relations extracted from
boxes an
existing labeled {\rgbd} dataset and a database of single 3D objects (IKEA in our case).
%
Then, given an input {\rgbd} image along with extracted boxes, the system will predict an initial label
for each box and estimate a list of suggested labels by reasoning on the box geometry and layout
using the trained classifiers.
%
In the annotation phase, user follows an intuitive "select then validate" scenario to select a box with most confident label
followed by either approving the label or picking alternative suggestion from a drop-down menu.
%
Based on the approved label, the system will automatically refine the geometry of box, re-estimate the label
for all remaining boxes and update the suggestion list.
%
This process is repeated until user is satisfy with the all the box labels.
%
The new labeled image is then added back to the existing labeled dataset with which the classifiers are re-trained.
%

The proposed system is different from traditional annotation tools in two aspects.
%
First, the nature that most indoor scenes are comprised of man-made objects inspires us to model the
scene using a collection of approximate boxy proxies (boxes for short) by exploiting the color and depth
data of {\rgbd} image.
%
We show that in addition to regular labels and segmentation masks that are provided by traditional annotation
tools, the representation using boxes also offers richer contextual information describes the scene structure in
the annotated data, including spatial arrangement, supporting hierarchy and mutual occlusion among objects,
which are proven to be useful for researches in scene understanding~\cite{}.
%
Second, in contrast to traditional annotation tools that completely rely on manual efforts to draw polygons on
object's outlines one at a time, we demonstrate that by leveraging the inferencing power of computer, the human
labor could be reduced dramatically.
%
Specifically, we incorporate a semi-supervised bootstrap learning algorithm to assist user annotating process.

%
Our goal is to provide users an easy and intuitive means to annotate objects in an indoor scene with minimal
manual efforts.
%
The key observation is that although it is effortless for humans to instantly recognize objects and reason
the structure in a scene, the major labor burden results from the tedious processes of manual labeling
and segmentation.
%
However, such burden could be significantly reduced by leveraging the strength of machines to perform
tasks
%

Specifically, the annotated data generated by our system would contain object labels, segmentation masks and
structural relationships including spatial arrangement, supporting hierarchy and mutual occlusion among objects,
which are proven to be tremendous useful for researches in scene understanding~\cite{}.
%

%the collection of labeled images.
%, especially for indoor scenes which covers many
%different object categories, there is few works emphasizing on an effective way to expand
%the collection of labeled images.

Although recent advances have demonstrated impressive gains in labeling accuracy~\cite{},
they are still far from a perfect solution.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% How do the existing works deal with this indoor scene labeling?
% What are the keys to robust scene labeling algorithm?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Most existing approaches in indoor scene labeling follow a common pipeline that comprises
two stages of training and labeling.
%
In the training stage, various image(and/or geometric) features are extracted from a set of
labeled data and are used to train statistic models among different object categories.
%
Then, in the labeling stage, objects' label in a given unlabeled scene are predicted based on
the evaluation of learned models.
%
Therefore, the key to a robust scene labeling algorithm is how to extract good features from
a sufficiently large and reliable set of labeled data that are used in the training stage.
%
While a majority of research efforts have focused on designing new features~\cite{}, the generation
of labeled data set still requires a tedious process of manual labeling.
%

Scene labeling, referring to the process of recognizing every object within a scenery image,
has made remarkable progress in the field of computer vision.
%
However, the majority of success lands in the outdoor scenes labeling~\cite{},
while leaving the labeling of indoor scenes remains a challenging task due to factors like
large variation in scene types and object categories, cluttering and occlusion
among objects, and poor illumination when capturing the indoor scene.
%
The key components to a reliable labeling algorithm are the employed features and large-scale labeled data
used in the training stage.
%

While a significant advances have been made in labeling outdoor scenes~\cite{},
recent research efforts have devoted to a more challenging scenario of indoor scenes~\cite{},
which might include large variation in scene types and object categories.

Labeling objects in a scene is a fundamental problem and has been extensively studied in
computer vision.
%
While the major success lands in the labeling of outdoor scenes~\cite{}, a large body
of work has recently focused on labeling objects in the indoor scenes~\cite{}.
%
Most existing approaches in indoor scene labeling follow a standard procedure.
%
Firstly, they apply a supervised learning algorithm on various {2D} image features
(e.g. SIFT, HOG,...etc) extracted from a set of labeled groundtruth scenes, followed by
an automatic labeling of unlabeled scenes using the trained model based on a
Markov random field (MRF)~\cite{} or conditional random field (CRF)~\cite{} formulation.
%
Recent efforts further demonstrate that by incorporating rich depth data acquired by the
widely available and affordable {\rgbd} sensors such as Microsoft Kinect into the learning stage
could significantly boost the performance in labeling accuracy~\cite{}.
%
%However, to the best of our knowledge, the labeling accuracy of 76.1\% on the NYU depth dataset~\cite{}
%reported by Ren~\etal~\cite{} is still far from perfection.
\fi


